Internal wave crystals

Geophysical fluids such as the ocean and atmosphere can be stratified: their density depends on the depth. As a consequence, they can host internal gravity waves that propagate in the bulk of the fluid, far from the surface. These waves can transport energy and momentum over large distances, thereby affecting large-scale circulation patterns, as well as the transport of heat, sediments, nutrients and pollutants in the ocean. When the density stratification is not uniform, internal waves can exhibit wave phenomena such as resonances, tunneling, and frequency-dependent transmissions. Spatially periodic density profiles formed by thermohaline staircases are commonly found in stratified fluids ranging from the Arctic Ocean to giant planet interiors, and can produce extended regions with periodically stratified fluid. Here, we report on the experimental observation of band gaps for internal gravity waves, ranges of frequencies over which the wave propagation is prohibited in the presence of a periodic stratification. We show the existence of surface states controlled by boundary conditions and discuss their topological origin. Our results suggest that energy transport can be profoundly affected by the presence of periodic stratifications in geophysical fluids ranging from Earth's oceans to gas giants.

==> media/Makefile <==
TIKZS := $(wildcard *.tikz)
TEXS := $(TIKZS:.tikz=.tex)
PDFS := $(TEXS:.tex=.pdf)

all: $(PDFS)

figures paper:

.PHONY: phony

phony:

%.pdf: %.tex phony
	latexmk -pdf -pdflatex="pdflatex" -use-make $<

%.tex: %.tikz
	sed 's/FILENAME\.tikz/$</g' tikz_template.tex > $@

table_definition_phases.tex:

clean:
	latexmk -C

cleanup:
	latexmk -c

